Applying Occam's Razor to Transformer-Based Dependency Parsing: What Works, What Doesn't, and What is Really Necessary

The introduction of pre-trained transformer-based contextualized word embeddings has led to considerable improvements in the accuracy of graph-based parsers for frameworks such as Universal Dependencies (UD). However, previous works differ in various dimensions, including their choice of pre-trained language models and whether they use LSTM layers. With the aims of disentangling the effects of these choices and identifying a simple yet widely applicable architecture, we introduce STEPS, a new modular graph-based dependency parser. Using STEPS, we perform a series of analyses on the UD corpora of a diverse set of languages. We find that the choice of pre-trained embeddings has by far the greatest impact on parser performance and identify XLM-R as a robust choice across the languages in our study. Adding LSTM layers provides no benefits when using transformer-based embeddings. A multi-task training setup outputting additional UD features may contort results. Taking these insights together, we propose a simple but widely applicable parser architecture and configuration, achieving new state-of-the-art results (in terms of LAS) for 10 out of 12 diverse languages.

==> sections/conclusion-old.tex <==
\section{Discussion and Conclusion}
\label{sec:conclusion}

In this paper, we have introduced STEPS, a new modular dependency parser which allows to easily perform experiments and principled architectural comparisons using a variety of settings.
Using STEPS, we have conducted a series of experiments in order to analyze how different implementation choices affect the performance of graph-based dependency parsing.

Our experimental results indicate that high-quality pre-trained token embeddings are by far the most crucial factor towards achieving high parsing accuracy.
In our case, the best results were achieved by using XLM-R, or, on some treebanks, language-specific BERT models.

Furthermore, we found that when using such embeddings, adding LSTM layers provides no additional benefit w.r.t. parsing accuracy or training time.
However, further architectural simplification in the form of an unfactorized parser architecture achieves slightly worse parsing accuracy and takes longer to train.
This suggests that in most cases, factorized models are preferable to unfactorized models when parsing UD.

Additionally, we have evaluated the impact of a multi-task setup in which the parsing system is also trained to predict UPOS and UFeats.
We have found that doing so tends to reduce parsing accuracy, an effect whose impact can be reduced by scaling down the loss of the tagging tasks.
However, to achieve ideal results across the parsing and tagging tasks, it may be preferable to use a pipeline model that handles them separately, or to use more sophisticated modes of interactions between the tasks, such as stack propagation \cite{zhang-weiss-2016-stack}.

Finally, we have also evaluated our system on the related task of Enhanced UD parsing. 
We found that our best model also achieves very good results in this setting, and that an unfactorized architecture becomes more competitive when parsing graphs, in line with previous results.

Overall, our results can be summed up as follows.
\begin{itemize}
	\item \textbf{What works:} High-quality language models such as XLM-R.
	\item \textbf{What doesn't:} Multi-task training.
	\item \textbf{What is not really necessary:} LSTM layers in addition to fine-tuned word embeddings.
\end{itemize}

Future work may address multilingual approaches such as the training setup used by UDify or more sophisticated models such as UDapter \cite{ustun-etal-2020-udapter}, which may be particularly beneficial in low-resource settings.
%\blue{Somehow phrase politely: useful for low resource langauges, but for high resource lang. one would probably always train a particular parser in practice (at least in settings where you know your input)}
Furthermore, it would be interesting to see if our results about biaffine achitectures also hold for non-syntactic tasks that have recently been framed as dependency parsing tasks, such as Named Entity Recognition \cite{yu-etal-2020-named} or Semantic Role Labeling \cite{shi-etal-2020-semantic}.
And finally, w.r.t. multi-task training, 

impact of parsing mtl on features, i.e., would completely separate models do better?

%LSTM:
%\stefantodo{It may potentially be possible that slightly better results could be achieved through more extensive hyperparameter tuning, should we mention this?}
%But here: solid system with reasonable amount of tuning is the goal ;)


